SofaMyRoom: a fast and multiplatform "shoebox" room simulator for binaural room impulse response dataset generation

This paper introduces a shoebox room simulator able to systematically generate synthetic datasets of binaural room impulse responses (BRIRs) given an arbitrary set of head-related transfer functions (HRTFs). The evaluation of machine hearing algorithms frequently requires BRIR datasets in order to simulate the acoustics of any environment. However, currently available solutions typically consider only HRTFs measured on dummy heads, which poorly characterize the high variability in spatial sound perception. Our solution allows to integrate a room impulse response (RIR) simulator with different HRTF sets represented in Spatially Oriented Format for Acoustics (SOFA). The source code and the compiled binaries for different operating systems allow to both advanced and non-expert users to benefit from our toolbox, see https://github.com/spatialaudiotools/sofamyroom/ .

==> parameter_table.tex <==
\begin{table}
	\centering
    \begin{adjustbox}{width=1\textwidth}
	
    \begin{tabular}{|l|l|p{4cm}|}
	\hline
	\multicolumn{3}{|c|}{Room Settings}\\\hline
	room.dimension & Room dimension [x,y,z] & double array \\ \hline
    room.humidity & Relative humidity (0,\dots,1) & double \\ \hline
    room.temperature & Room temperature (Celsius) & double \\\hline
    
	\multicolumn{3}{|c|}{Surface Absorption and Diffusion Coefficients}\\\hline
	room.surface.frequency & Frequency bands & double array\\ \hline
	room.surface.absorption & Absorption coefficients & double array \\ \hline
	room.surface.diffusion & Diffusion coefficients & double array \\\hline
	
	\multicolumn{3}{|c|}{Simulation Options}\\\hline
	options.fs & Sampling frequency [Hz] & integer \\ \hline
	options.responseduration & Duration of the impulse response [s] & double\\ \hline
	options.bandsperoctave & Simulation frequency accuracy (1, 2, 3, or 4 bands/octave) & integer \\ \hline
	options.referencefrequency & Reference frequency for frequency octaves [Hz] & double \\ \hline
	options.airabsorption & Apply air absorption & boolean \\ \hline
	options.distanceattenuation & Apply distance attenuation & boolean \\ \hline
	options.subsampleaccuracy & Apply subsample accuracy & boolean \\ \hline
	options.highpasscutoff & 3dB frequency of high-pass filter & boolean \\ \hline
	options.verbose & Print status messages & boolean \\\hline
	
	\multicolumn{3}{|c|}{Specular Reflections Simulation Options}\\\hline
	options.simulatespecular & Simulate specular reflections & boolean\\ \hline
	options.reflectionorder & Maximum specular reflection order [x,y,z] & integer arrray \\\hline
	
	\multicolumn{3}{|c|}{Diffuse reflections simulation options}\\\hline
	options.simulatediffuse & Simulate diffuse reflections & boolean \\ \hline
	options.numberofrays & Number of rays in simulation $(20\cdot K^2)$ & integer \\ \hline
	options.diffusetimestep & Time resolution in diffuse energy histogram [s] & double \\ \hline
	options.rayenergyfloordB & Ray energy threshold with respect to initial energy [dB] & double\\ \hline
	options.uncorrelatednoise & Use uncorrelated poisson arrivals & boolean \\\hline
	
	\multicolumn{3}{|c|}{Output Options}\\\hline
	options.outputname & Name of the output file & string \\ \hline
	options.saveaswav & Format of the ouput file & boolean \\\hline
	
	\multicolumn{3}{|c|}{Source Definitions}\\\hline
	source($n$).location & Location of source [x,y,z] (meters) & double array \\ \hline
	source($n$).orientation & Orientation of source (yaw, pitch, roll) [degrees] & double array \\ \hline
	source($n$).description & Source type & {omnidirectional, cardioid, subcardioid, hypercardiod, supercardioid, unidirectional, bidirectional, dipole, hemisphere}\\\hline
	
	\multicolumn{3}{|c|}{Receiver Definitions}\\\hline
	receiver($n$).location & Location of receiver (x, y, z) (meters) & \\ \hline
	receiver($n$).orientation & Orientation of receiver (yaw, pitch, roll) (degrees) &\\ \hline
	receiver($n$).description & Receiver type &\\\hline
    \end{tabular}
    \end{adjustbox}
	\caption{Full list of SofaMyRoom parameters.}
	\label{tab:params}
\end{table}
